Fairness in Ranking under Uncertainty

Fairness has emerged as an important consideration in algorithmic decision-making. Unfairness occurs when an agent with higher merit obtains a worse outcome than an agent with lower merit. Our central point is that a primary cause of unfairness is uncertainty. A principal or algorithm making decisions never has access to the agents' true merit, and instead uses proxy features that only imperfectly predict merit (e.g., GPA, star ratings, recommendation letters). None of these ever fully capture an agent's merit; yet existing approaches have mostly been defining fairness notions directly based on observed features and outcomes. Our primary point is that it is more principled to acknowledge and model the uncertainty explicitly. The role of observed features is to give rise to a posterior distribution of the agents' merits. We use this viewpoint to define a notion of approximate fairness in ranking. We call an algorithm $\phi$-fair (for $\phi \in [0,1]$) if it has the following property for all agents $x$ and all $k$: if agent $x$ is among the top $k$ agents with respect to merit with probability at least $\rho$ (according to the posterior merit distribution), then the algorithm places the agent among the top $k$ agents in its ranking with probability at least $\phi \rho$. We show how to compute rankings that optimally trade off approximate fairness against utility to the principal. In addition to the theoretical characterization, we present an empirical analysis of the potential impact of the approach in simulation studies. For real-world validation, we applied the approach in the context of a paper recommendation system that we built and fielded at the KDD 2020 conference.

==> reviewer_comments_kdd.tex <==
reviewer 1:

In general, I found the paper interesting to read. In my opinion, the proposed axiomatic approach to fairness in rankings properly handles the inherent uncertainty existing in several real-world scenarios (e.g., hiring). Ranking an item in the top-k according to the probability of the item's merit being among the top-k is natural and the theoretical assumptions and results seem well-justified by the authors.

The real-world experiment is interesting, however, the experimental section as a whole is not particularly insightful. The result presented in Figure 2 comparing the utility between the mixed policy and the LP-based policy is somewhat expected. Perhaps it would have been more interesting to explore a synthetic experimental setting instead, in order to be able to further analyze when the performance of the two policies gets greater or smaller. Also, the results in Table 1 don't seem to convey a strong message since several "engagement" metrics are presented with some of them showing stronger engagement for the utility-maximizing policy (e.g., Add to calendar) and others showing stronger engagement for the Thomson-Sampling fair policy (e.g., Read PDF, Add Bookmark). Finally, a problem that would appear in practice is the estimation of the merit distribution $\Gamma$. In both Sections 4 & 5, the authors make certain assumptions in order to be able to generate that distribution but it's not perfectly clear how those merits can be estimated in more general settings.

In terms of writing, I found the paper very well-written. I only have some minor comments:
1) In Section 3.3, I found the example a little weird. The authors write that "... the distribution places equal probability on each of the URM candidates having merit $1+\epsilon$". Is it natural to assume that? In reality, I would expect that a merit estimator would probably underestimate the merit of all under-represented individuals instead of knowing its true value but don't knowing on which specific individual to attribute it. In that sense, even though I understand the point the authors want to make in this section, the example itself was a little confusing to read.
2) In Section 4, when describing the generative model of the rating, it would have been helpful to provide some intuition regarding the assumptions, in order for the reader to be able to understand how realistic that setting is.

Overall, I think this paper provides an interesting perspective and formulation of fairness in rankings and the method/results presented by the authors are important from a theoretical perspective. Also, I found the quality of the writing very good. However, I think the experimental part was somewhat simplistic and it could have been more insightful. Therefore, I am neutral about the paper's acceptance.


reviewer 2:

Strengths:
- The experimental evaluation goes beyond readily-available datasets, and includes a field experiment
- Uncertainty is an important concept in measurements of merit, and the formalization of it seems technically sound and applicable in a broad range of scenarios
- The discussion on distributing the cost of unfairness between the ones affected and the principal is very promising. The formalization of this concept seems well executed.

Weaknesses:
- The experimental evaluation lacks comparisons with relevant prior work on fair ranking.
- The field experiment lacks details about how it was conducted.
- The assumption that fairness and utility necessarily have to be traded against one another does not always hold, see recent work by Zehlike et al. [2]. Zehlike el al. show that when bias affects the score distribution differently across groups, obtaining fairer results increases utility. Group fairness metrics are justified precisely because there is uncertainty about measures of merit and their comparability across groups.
- In this paper, uncertainty is mostly treated as "not enough data of the minorities", instead of "measurements of merits experience different biases across groups, and usually such bias is higher for minorities". The paper says that the distribution Γ can be inferred with Bayesian inference procedures and that the principal has an incentive to gather more information on the minority. While this is a necessary step, it still means that Γ will be inferred from observations that stem from the same biased merit measures. The paper does not say anything on the uncertainty of merits because of biased observation processes. It would be good to include a discussion of this limitation.
- The discussion states that the framework should rather be used in e-commerce and the lot, and not so much in contexts of admissions, but then in the rest of the paper several examples relate to cases of hiring scenarios. It would be good to change these examples then.

Minor:
- There is no Figure 3(a)
- [1] is an important work on individual fairness and should be featured in related work

Missing References:
[1] Lahoti, Preethi, Krishna P. Gummadi, and Gerhard Weikum. "Operationalizing individual fairness with pairwise fair representations." Proceedings of VLDB Endowment 13 (4), 506–518 (2019).
[2] Zehlike, Meike, and Carlos Castillo. "Reducing disparate exposure in ranking: A learning to rank approach." Proceedings of The Web Conference 2020. 2020.

reviewer 3:

+ This paper studies the fair ranking problem in the presence of uncertainty about the agent's merits. This topic is very interesting and important.
+ Following the defined $\phi$-fairness, the paper explores the trade-off of utility and fairness. Then it develops an optimization solution to find a distribution subject to the fairness constraints. The formulation and solution seem well and sound.

- My major concern is the intuitive notion of $\phi$-fairness. It does be similar to individual fairness where similar users obtain similar output. But the key fact, two users from different demographic groups, is missing. It would be convincing if the connection between individual fairness and $\phi$-fairness is more clearly presented.
- I have small concerns on experiments. In the experiment of MovieLens, the performance of fairness is unclear. I am also curious how fairness is evaluated in MovieLens dataset. There is lack of baseline methods from existing research in the experiments.

reviewer 4:
This paper presents an axiomatic approach towards fairness in ranking under uncertainty. The paper is well organized and well presented. However, the major flaws are in the experimental sections. (1) the dataset used in the real-world experiments is not clear; (2) which evaluation matrices are used to measure fairness, accuracy, and trade-off between those? (3) there is no clue to find out the baseline methods to use to compare with the proposed method. (4) the reproducibility is low and details of experiments, such as hyperparameter tuning, are not given. Although a lot of information are given in the experiment section, experiments overall are not extensive and hence it is hard to convince reviewers with the effectiveness and efficiency of the proposed method.
Go Back
